MBD: A Model-Based Debiasing Framework Across User, Content, and Model Dimensions

Modern recommendation systems rank candidates by aggregating multiple behavioral signals through a value model. However, many commonly used signals are inherently affected by heterogeneous biases. For example, watch time naturally favors long-form content, loop rate favors short - form content, and comment probability favors videos over images. Such biases introduce two critical issues: (1) value model scores may be systematically misaligned with users' relative preferences - for instance, a seemingly low absolute like probability may represent exceptionally strong interest for a user who rarely engages; and (2) changes in value modeling rules can trigger abrupt and undesirable ecosystem shifts. In this work, we ask a fundamental question: can biased behavioral signals be systematically transformed into unbiased signals, under a user - defined notion of ``unbiasedness'', that are both personalized and adaptive? We propose a general, model-based debiasing (MBD) framework that addresses this challenge by augmenting it with distributional modeling. By conditioning on a flexible subset of features (partial feature set), we explicitly estimate the contextual mean and variance of the engagement distribution for arbitrary cohorts (e.g., specific video lengths or user regions) directly alongside the main prediction. This integration allows the framework to convert biased raw signals into unbiased representations, enabling the construction of higher-level, calibrated signals (such as percentiles or z - scores) suitable for the value model. Importantly, the definition of unbiasedness is flexible and controllable, allowing the system to adapt to different personalization objectives and modeling preferences. Crucially, this is implemented as a lightweight, built-in branch of the existing MTML ranking model, requiring no separate serving infrastructure.

==> symbol.tex <==
%\newcommand{\cX}{\mathcal{X}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cS}{\mathcal{S}}
% \newcommand{\cP}{\mathcal{P}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
% \newcommand{\cG}{\mathcal{G}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cC}{\mathcal{C}}

\newcommand{\bR}{\mathbb{R}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bP}{\mathbb{P}}

\newcommand{\wtU}{\widetilde{U}}
\newcommand{\wtW}{\widetilde{W}}
\newcommand{\wtH}{\widetilde{H}}
\newcommand{\wtL}{\widetilde{L}}
\newcommand{\wtbeta}{\widetilde{\beta}}
\newcommand{\wtcF}{\widetilde{\cF}}
\newcommand{\wtcA}{\widetilde{\cA}}
\newcommand{\wbcup}{\mathop{\bigcup}\displaylimits}
\newcommand{\wbcap}{\mathop{\bigcap}\displaylimits}


\newcommand{\dom}{{\bf dom}\,}
\newcommand{\Tra}{^{\sf T}} % Transpose
\newcommand{\Inv}{^{-1}} % Inverse
\def\vec{\mathop{\rm vec}\nolimits}
%\newcommand{\diag}{\mathop{\rm diag}\nolimits}
%\newcommand{\tr}{\operatorname{tr}} % Trace
\newcommand{\epi}{\operatorname{epi}} % epigraph
\newcommand{\V}[1]{{\bm{\mathbf{\MakeLowercase{#1}}}}} % vector
\newcommand{\VE}[2]{\MakeLowercase{#1}_{#2}} % vector element
\newcommand{\Vn}[2]{\V{#1}^{(#2)}} % n-th vector
\newcommand{\Vtilde}[1]{{\bm{\tilde \mathbf{\MakeLowercase{#1}}}}} % vector
\newcommand{\Vhat}[1]{{\bm{\hat \mathbf{\MakeLowercase{#1}}}}} % vector
\newcommand{\VtildeE}[2]{\tilde{\MakeLowercase{#1}}_{#2}} % vector element
\newcommand{\M}[1]{{\bm{\mathbf{\MakeUppercase{#1}}}}} % matrix
\newcommand{\ME}[2]{\MakeLowercase{#1}_{#2}} % matrix element
\newcommand{\Mtilde}[1]{{\bm{\tilde \mathbf{\MakeUppercase{#1}}}}} % matrix
\newcommand{\Mbar}[1]{{\bm{\bar \mathbf{\MakeUppercase{#1}}}}} % matrix
\newcommand{\Mn}[2]{\M{#1}^{(#2)}} % n-th matrix
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\argminE}{\mathop{\mathrm{argmin}}} 

\newcommand{\mmts}{\text{MMTS}}
\newcommand{\cmcp}{\text{CMCPR}}
\newcommand{\mw}{\textit{m}-\text{type worker}}
\newcommand{\app}[1]{\text{applicant}}
\newcommand{\com}[1]{\text{company}}
\newcommand{\br}{\mathfrak{R}(T)}

\newcommand{\fab}{\text{FAB}}
\newcommand{\fats}{\text{FATS}}
\newcommand{\ffats}{\text{F-FATS}}
\newcommand{\pfats}{\text{P-FATS}}

==> symbol_old.tex <==
\renewcommand{\P}{\mathbb{P}}
\newcommand{\PSD}{\mathbb{S}_{++}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\btilK}{\boldsymbol{\tilde{K}}}
\newcommand{\btilG}{\boldsymbol{\tilde{G}}}
\newcommand{\tilsigma}{\tilde{\sigma}}
\newcommand{\bhatK}{\boldsymbol{\hat{K}}}
\newcommand{\bhatG}{\boldsymbol{\widehat{G}}}
\newcommand{\bhatM}{\boldsymbol{\widehat{M}}}
\newcommand{\bhatP}{\boldsymbol{\widehat{P}}}
\newcommand{\bhatH}{\boldsymbol{\hat{H}}}
\newcommand{\pinv}{\dagger}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\xstar}{x^{\star}}
\newcommand{\bxstar}{\bx^{\star}}
\newcommand{\bxstarfixed}{\bx^{\star \, \mathrm{(fixed)}}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\boldeta}{\boldsymbol{\eta}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bl}{\boldsymbol{l}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bhatC}{\boldsymbol{\wh{C}}}
\newcommand{\bhM}{\boldsymbol{\wh{M}}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\btilM}{\boldsymbol{\tilde{M}}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\btilD}{\boldsymbol{\tilde{D}}}
\newcommand{\bhG}{\boldsymbol{\wh{G}}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\sK}{\mathcal{K}}
\newcommand{\sS}{\mathcal{S}}
\newcommand{\sI}{\mathcal{I}}
\newcommand{\bhatY}{\boldsymbol{\hat{Y}}}
\newcommand{\bbarW}{\boldsymbol{\bar{W}}}
\newcommand{\bbary}{\boldsymbol{\bar{y}}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\btilz}{\boldsymbol{\tilde{z}}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bbarZ}{\boldsymbol{\bar{Z}}}
\newcommand{\bbarz}{\boldsymbol{\bar{z}}}
\newcommand{\bhatZ}{\boldsymbol{\hat{Z}}}
\newcommand{\bhatz}{\boldsymbol{\hat{z}}}
\newcommand{\bhatx}{\boldsymbol{\hat{x}}}
\newcommand{\haty}{\hat{y}}
\newcommand{\ystar}{y^{\star}}
\newcommand{\lambdah}{\hat{\lambda}}
\newcommand{\lambdawh}{\widehat{\lambda}}
\newcommand{\dhat}{\widehat{d}}
\newcommand{\lambdabar}{\bar{\lambda}}
\newcommand{\Lambdah}{\hat{\Lambda}}
\newcommand{\barz}{\bar{z}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bbarS}{\boldsymbol{\bar{S}}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\btilw}{\boldsymbol{\tilde{w}}}
\newcommand{\brr}{\boldsymbol{r}}
\newcommand{\bbarw}{\boldsymbol{\bar{w}}}
\newcommand{\bbarwstar}{\boldsymbol{\bar{w}}^{\star}}
\newcommand{\barw}{\bar{w}}
\newcommand{\bhatw}{\wh{\boldsymbol{w}}}
\newcommand{\bhatW}{\boldsymbol{\hat{W}}}
\newcommand{\bhatwl}{\bhatw_{\lambda}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\btilW}{\boldsymbol{\tilde{W}}}
\newcommand{\bWstar}{\boldsymbol{W^{\star}}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\sA}{\mathcal{A}}
\newcommand{\sP}{\mathcal{P}}
\newcommand{\sC}{\mathcal{C}}
\newcommand{\sL}{\mathcal{L}}
\newcommand{\sN}{\mathcal{N}}
\newcommand{\sM}{\mathcal{M}}
\newcommand{\sB}{\mathcal{B}}
\newcommand{\shatB}{\wh{\mathcal{B}}}
\newcommand{\shatBli}{\wh{\mathcal{B}}_{\lambda,i}}
\newcommand{\shatBlj}{\wh{\mathcal{B}}_{\lambda,j}}
\newcommand{\shatBlI}{\wh{\mathcal{B}}_{\lambda,I}}
\newcommand{\sBstar}{\mathcal{B}^{\star}}
\newcommand{\sBstarli}{\mathcal{B}_{\lambda,i}}
\newcommand{\sBstarlj}{\mathcal{B}^{\star}_{\lambda,j}}
\newcommand{\sBstarlI}{\mathcal{B}^{\star}_{\lambda,I}}
\newcommand{\sEstar}{\mathcal{E}^{\star}}
\newcommand{\sEstarli}{\mathcal{E}_{\lambda,i}}
\newcommand{\sEstarlj}{\mathcal{E}^{\star}_{\lambda,j}}
\newcommand{\sEstarlI}{\mathcal{E}^{\star}_{\lambda,I}}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sE}{\mathcal{E}}
\newcommand{\sT}{\mathcal{T}}
\newcommand{\sD}{\mathcal{D}}
\newcommand{\sF}{\mathcal{F}}
\newcommand{\sH}{\mathcal{H}}
\newcommand{\sG}{\mathcal{G}}
\newcommand{\sW}{\mathcal{W}}
\newcommand{\sZ}{\mathcal{Z}}
\newcommand{\barg}{\bar{g}}
\newcommand{\sbarZ}{\bar{\mathcal{Z}}}
\newcommand{\fbag}{\bold{F}}
\newcommand{\ind}[1]{\mathbb{I}\left\{ #1 \right\}}
\newcommand{\phih}{\hat{\phi}}
\newcommand{\bphi}{\boldsymbol{\phi}}


\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\rank}{rank}
\newcommand{\var}[1]{\underset{#1}{\operatorname{Var}}}


\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\fY}{\field{Y}}
\newcommand{\fX}{\field{X}}
\newcommand{\fH}{\field{H}}

\newcommand{\R}{\field{R}}
\newcommand{\Nat}{\field{N}}
\newcommand{\Var}{\mathrm{Var}}
\renewcommand{\Im}{\mathrm{Im}}

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}


\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bvartheta}{\boldsymbol{\vartheta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bargamma}{\bar{\gamma}}
\newcommand{\bvarepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\bbartheta}{\boldsymbol{\bar{\theta}}}
\newcommand\theset[2]{ \left\{ {#1} \,:\, {#2} \right\} }
\newcommand\inn[2]{ \left\langle {#1} \,,\, {#2} \right\rangle }
\newcommand\RE[2]{ D\left({#1} \| {#2}\right) }
\newcommand\I[1]{ \mathbb{I}\left\{{#1}\right\} }
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\diag}{\operatorname{diag}}

\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\sgn}{\mbox{\sc sgn}}
\newcommand{\scI}{\mathcal{I}}
\newcommand{\scO}{\mathcal{O}}
\newcommand{\scR}{\mathcal{R}}
\newcommand{\schatR}{\wh{\mathcal{R}}}
\newcommand{\sctilO}{\mathcal{\tilde{O}}}
\newcommand{\tilTheta}{\tilde{\Theta}}

\newcommand{\dt}{\displaystyle}
\renewcommand{\ss}{\subseteq}
\newcommand{\wh}{\widehat}
\newcommand{\ve}{\varepsilon}
\newcommand{\bve}{\boldsymbol{\varepsilon}}
\newcommand{\hlambda}{\wh{\lambda}}
\newcommand{\yhat}{\wh{y}}
\newcommand{\fhat}{\wh{f}}
\newcommand{\bhatg}{\wh{\boldsymbol{g}}}

\newcommand{\hDelta}{\wh{\Delta}}
\newcommand{\hdelta}{\wh{\delta}}
\newcommand{\spin}{\{-1,+1\}}


\newcommand{\reals}{\mathbb{R}}
\newcommand{\sign}{{\rm sign}}

\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\tp}{^{\top}}
\newcommand{\ip}[1]{\left\langle #1 \right\rangle}
\newcommand{\ME}[1]{\underset{#1}{\mathbb{E}}}
\newcommand{\MEbr}[2]{\underset{#1}{\mathbb{E}}\left[ #2 \right]}
%\newcommand{\ME}[1]{\mathbb{E}_{#1}}
%\newcommand{\MEh}[1]{\underset{#1}{\hat{\mathbb{E}}}}
\newcommand{\Sloo}{S^{\backslash i}}
\newcommand{\Sdel}{S^{\backslash i}}
\newcommand{\Srep}{{S^{(i)}}}
\newcommand{\Srept}{{S^{(t)}}}
\newcommand{\Srepk}{{S^{(k)}}}
\newcommand{\Stilrep}{S^{'(i)}}
\newcommand{\repi}{^{(i)}}
\newcommand{\repj}{^{(j)}}
\newcommand{\repk}{^{(k)}}
\newcommand{\repkj}{^{(k,j)}}
\newcommand{\repik}{^{(i \rightarrow k)}}
\newcommand{\loo}{_{\Sloo}}
\newcommand{\looi}{^{\backslash i}}
\newcommand{\looiinv}{^{\backslash i~ -1}}
\newcommand{\fhtlold}{f^{htl}_{S}}
\newcommand{\fhtl}{f^{htl'}_{S}}
\newcommand{\fhtlloo}{f^{htl'}\loo}
\newcommand{\fh}{\hat{f}}
\newcommand{\Riskh}{\wh{R}}
\newcommand{\Rhat}{\wh{R}}
\newcommand{\Rhatl}{\wh{R}_{\lambda}}
\newcommand{\Rhatli}{\wh{R}_{\lambda,i}}
\newcommand{\Rhatlj}{\wh{R}_{\lambda,j}}
\newcommand{\Rl}{R_{\lambda}}
\newcommand{\Rstar}{R^{\star}}
\newcommand{\Rstarl}{R^{\star}_{\lambda}}
\newcommand{\Rstarli}{R^{\star}_{\lambda,i}}
\newcommand{\Rstarlj}{R^{\star}_{\lambda,j}}
%\newcommand{\Risk}[1]{\underset{#1}{R}}
\newcommand{\Risk}{R}
\newcommand{\Riskloo}{R^{\textnormal{~loo}}}
\newcommand{\Riskhloo}{\hat{R}^{\textnormal{~loo}}}
\newcommand{\Rad}{\mathfrak{R}}
\newcommand{\Radh}{\widehat{\mathfrak{R}}}
\newcommand{\Radabs}{\mathfrak{R}^{|\cdot|}}
\newcommand{\Radhabs}{\hat{\mathfrak{R}}^{|\cdot|}}
\newcommand{\Gau}{\mathfrak{G}}
\newcommand{\Gauh}{\hat{\mathfrak{G}}}
\newcommand{\dm}[1]{\mathrm{dim }\left(#1\right)}
\newcommand{\distas}[1]{\mathbin{\overset{#1}{\sim}}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\fbayes}{g^{\star}}
\newcommand{\gstar}{g^{\star}}
\newcommand{\pstar}{p^{\star}}
\newcommand{\etastar}{\eta^{\star}}
\newcommand{\iid}{\mathrm{iid}}
\newcommand{\distasiid}{\distas{\iid}}


%\renewcommand{\sup}[1]{\underset{#1}{\operatorname{sup~}}}
\DeclareMathOperator*{\esssup}{ess~\,sup}
\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\V}{\mathbb{V}}
\DeclareMathOperator*{\supp}{\mathrm{supp}}
\newcommand{\Ei}{\mathbb{E}_{-i}}
\newcommand{\Ech}{\mathbb{E}}
\newcommand{\EfixS}[1]{\E\br{#1 \;\middle|\; S}}

\newcommand{\supbr}[2]{ \sup{#1}\left[#2\right] }
\newcommand{\hsrc}{h^{\mathrm{src}}}
\newcommand{\src}{^{\mathrm{src}}}
\newcommand{\trg}{^{\mathrm{trg}}}
\newcommand{\usrc}{^{\mathrm{s}}}
\newcommand{\utrg}{^{\mathrm{t}}}
\newcommand{\usrctrg}{^{\mathrm{st}}}
\newcommand{\bwsrc}{\bw^{\mathrm{\schape{src}}}}
\newcommand{\htrg}{h^{\mathrm{trg}}}
\newcommand{\ones}{\boldsymbol{1}}
\newcommand{\one}{\mathds{1}}

\newcommand{\barX}{\bar{X}}
\newcommand{\T}[1]{\hbox{\bfseries{\scshape{t}}}_C\left\{#1\right\}}

\def\Plus{\texttt{+}}
\def\Minus{\texttt{-}}
\def\Ref{\texttt{ref}}
\def\dis{\texttt{dis}}
\def\pair{\texttt{p}}

%\newtheoremstyle{named}{}{}{\itshape}{}{\bfseries}{}{.5em}{\thmnote{#3.}#1}
%\theoremstyle{named}
%\newtheorem*{nameddef}{}

\declaretheoremstyle[
spaceabove=\topsep, spacebelow=\topsep,
headfont=\normalfont\bfseries,
notefont=\bfseries, notebraces={}{},
bodyfont=\normalfont\itshape,
postheadspace=0.5em,
name={\ignorespaces},
numbered=no,
headpunct=.]
{mystyle}
\declaretheorem[style=mystyle]{nameddef}

\newcommand{\nnst}{{\pi_t{(\boldsymbol{x}_t)}}}
\newcommand{\nnsi}{{\pi_t{(\boldsymbol{x}_i)}}}
\newcommand{\nnstarg}[1]{{\pi_{t}{(\boldsymbol{x}_t, #1)}}}
\newcommand{\nnstX}{{\pi_t{(X_t)}}}

\newcommand{\Ntot}{N^\textsc{tot}}
\newcommand{\Stot}{S^\textsc{tot}}

\newcommand{\lbr}{\left[}
\newcommand{\rbr}{\left]}
\newcommand{\phat}{\widehat{p}}
\newcommand{\rloc}{r^{\mathrm{\tiny \textsc{loc}}}}
\newcommand{\rglob}{r^{\mathrm{\tiny \textsc{glb}}}}
%\newcommand{\safebeta}{\max\{1,\beta\}}
\newcommand{\safebeta}{1 \vee \beta}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\lmin}{\lambda_{\mathrm{min}}}
\newcommand{\lminh}{\widehat{\lambda}_{\mathrm{min}}}
\newcommand{\lmax}{\lambda_{\mathrm{max}}}
\newcommand{\lmini}{\lambda_{\mathrm{min},i}}
\newcommand{\lwhmax}{\wh{\lambda}_{\mathrm{max}}}
\newcommand{\lwhmaxi}{\wh{\lambda}_{\mathrm{max},i}}
\newcommand{\smin}{s_{\mathrm{min}}}
\newcommand{\smax}{s_{\mathrm{max}}}
\newcommand{\vol}{\mathrm{vol}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\kl}{\mathrm{kl}}
\newcommand{\Ep}{E_{{\pi}}}
\newcommand{\Bp}{B_{{\pi}}}
\newcommand{\subd}{s}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\mustar}{\mu^{\star}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bhSigma}{\boldsymbol{\wh{\Sigma}}}
\newcommand{\eps}{\epsilon}
\newcommand{\lb}{\lambdabar}
%\newcommand{\ceil}[1]{\left[#1\right]}
\newcommand{\phase}{N_i}
\newcommand{\tupd}{{t+\frac{1}{2}}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\diam}{\mathrm{diam}}
\newcommand{\delstar}{\nabla^\star}
%\newcommand{\nablatil}{\tilde{\nabla}}
\newcommand{\deltil}{\widetilde{\nabla}}
\newcommand{\nablahat}{\wh{\nabla}}
\newcommand{\phalf}{^{\frac{1}{2}}}
\newcommand{\ph}{^{\frac{1}{2}}}
\newcommand{\minph}{^{-\frac{1}{2}}}

\newcommand{\pr}[1]{\left( #1 \right)}
\newcommand{\br}[1]{\left[ #1 \right]}
\newcommand{\cbr}[1]{\left\{ #1 \right\}}
\newcommand{\abs}[1]{\left|#1\right|}

\newcommand{\lf}{\left}
\newcommand{\rt}{\right}
\newcommand{\pred}{\mathrm{pred}}
\newcommand{\regret}{\mathrm{Reg}}
\newcommand{\seq}{\mathrm{Seq}}
\newcommand{\kgrad}{k^{\mathrm{grad}}}
\newcommand{\cover}{\mathrm{Cover}}
\newcommand{\sqrtrisk}{r}

\newcommand{\mixsrcloss}{\bar{L}}
\newcommand{\srcloss}{L\src}
\newcommand{\Riskinit}{\Risk(\bw_1)}
\newcommand{\Riskend}{r}
\newcommand{\GD}{\text{\scshape{gd}}}
\newcommand{\leaves}{\mathrm{leaves}}

%\newcommand{\ps}{p_{S,\gamma}}
%\newcommand{\prior}{p^0_{\gamma}}
%\newcommand{\Zs}{Z_{S,\gamma}}
%\newcommand{\Zprior}{Z^0_{\gamma}}

\newcommand{\psbeta}{\wh{p}_S^{\beta}}
\newcommand{\pscond}{p_{S, r}}
\newcommand{\psrepcond}{p_{\Srep, r}}
\newcommand{\pscondA}{p_{S, A}}
\newcommand{\psrepcondA}{p_{\Srep, A}}
\newcommand{\qcond}{q_{r}}
\newcommand{\psB}{p_{S,\sB}}
\newcommand{\qs}{q_{S}}
\newcommand{\qsB}{q_{S,\sB}}
\newcommand{\psrep}{p_{\Srep}}
\newcommand{\prior}{p^0}
\newcommand{\Zs}{Z_{S}}
\newcommand{\Zprior}{Z^0}
%\newcommand{\deff}{d^{\mathrm{eff}}_S(\lambda)}
\newcommand{\deff}{d^{\star}}
\newcommand{\deffIS}{d^{\mathrm{eff}}_S(\lambda,I_S)}
\newcommand{\deffbar}{\bar{d}_{\mathrm{eff}}}


\newcommand{\wt}{\widetilde}
\newcommand{\defO}{\stackrel{\scO}{=}}

\newcommand{\defOtilde}{\stackrel{\wt{\scO}}{=}}
\newcommand{\Erf}{\mathrm{Erf}}
\newcommand{\egen}{\Delta^{\mathrm{gen}}}
%\newcommand{\excess}{\Delta^{\mathrm{ex}}}
\newcommand{\excess}{\Delta}
\newcommand{\excesshat}{\wh{\Delta}^{\mathrm{ex}}}
\newcommand{\veapprox}{\varepsilon_{\mathrm{approx}}}
\newcommand{\velb}{\varepsilon_{\mathrm{lb}}}
\newcommand{\veub}{\varepsilon_{\mathrm{ub}}}
\newcommand{\erf}{\mathrm{erf}}
\newcommand{\glob}{^{\mathrm{\scshape{glob}}}}
\newcommand{\loc}{^{\mathrm{\scshape{loc}}}}
\newcommand{\subopt}{^{\mathrm{\scshape{subopt}}}}
\newcommand{\hcross}{h^{\mathrm{cross}}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}

\newcommand{\wstar}{w^{\star}}
\newcommand{\bwstar}{\bw^{\star}}
\newcommand{\bwstartp}{\bw^{\star \top}}
\newcommand{\bwstarl}{\bw^{\star}_{\lambda}}
\newcommand{\bwstarli}{\bw^{\star}_{\lambda, i}}
\newcommand{\bwstarlj}{\bw^{\star}_{\lambda, j}}
\newcommand{\bwstarlI}{\bw^{\star}_{\lambda, I}}
\newcommand{\bHstar}{\boldsymbol{H}^{\star}}
\newcommand{\bHstarl}{\boldsymbol{H}^{\star}_{\lambda}}
\newcommand{\bHstarli}{\boldsymbol{H}^{\star}_{\lambda,i}}
\newcommand{\bHstarI}{\boldsymbol{H}^{\star}_{I}}
\newcommand{\bHstarlI}{\boldsymbol{H}^{\star}_{\lambda,I}}
\newcommand{\bHstarlj}{\boldsymbol{H}^{\star}_{\lambda,j}}
\newcommand{\bHstarlhalf}{\boldsymbol{H}^{\star \frac{1}{2}}_{\lambda}}
\newcommand{\bHstarlinv}{\boldsymbol{H}^{\star -1}_{\lambda}}
\newcommand{\bHstarlIinv}{\boldsymbol{H}^{\star -1}_{\lambda,I}}
\newcommand{\pistar}{\pi^{\star}}
\newcommand{\pihat}{\wh{\pi}}
\newcommand{\ellipse}{\sE^{\star}_{\gamma}}
\newcommand{\sqrtTemp}{\nicefrac{1}{\sqrt{\gamma}}}
\newcommand{\Temp}{\nicefrac{1}{\gamma}}
% \newcommand{\sqrtTemp}{\sqrt{\tau}}
% \newcommand{\Temp}{\tau}
\newcommand{\Lip}{\Delta}
\newcommand{\Lipi}{L^{\star}_i}
\newcommand{\Phat}{\widehat{P}}
\newcommand{\comment}[2]{{\color{blue} (#1: #2)}}
\newcommand{\mincomp}{\sC^{\star}}


\newcommand{\barell}{\bar{\ell}}
\newcommand{\nash}{\boldsymbol{\bar{x}}^{\star}}
% \newcommand{\comp}{\boldsymbol{\bar{z}}}
% \newcommand{\compx}{z}
% \newcommand{\bcompx}{\bz}

\newcommand{\comp}{\boldsymbol{\bar{x}^{\star}}}
\newcommand{\compx}{x^{\star}}
\newcommand{\bcompx}{\bxstar}

\newcommand{\nashfixed}{\boldsymbol{\bar{x}}^{\star \, \mathrm{(fixed)}}}
\newcommand{\nashi}{\boldsymbol{\bar{x}}^{\star}_i}
\newcommand{\bbarx}{\boldsymbol{\bar{x}}}
\newcommand{\bbarxstar}{\boldsymbol{\bar{x}^{\star}}}
\newcommand{\bbark}{\boldsymbol{\bar{k}}}
\newcommand{\sstar}{s^{\star}}
\newcommand{\Sstar}{S^{\star}}
\newcommand{\hR}{\hat{R}}
\newcommand{\vh}{\hat{v}}
\newcommand{\IS}{\mathrm{IS}}
\newcommand{\CVlambda}{\mathrm{CV-}\lambda}
\newcommand{\Vdel}{V_{\mathrm{del}}}
\newcommand{\Vhatdel}{\widehat{V}^{\, \mathrm{del}}}
\newcommand{\Vhatdeli}{\widehat{V}^{\backslash i}}
\newcommand{\Vhatdell}{\widehat{V}^{\backslash l}}
\newcommand{\Vrep}{V_{\mathrm{rep}}}
%\newcommand{\Vtilrep}{\widetilde{V}_{\mathrm{rep}}}
\newcommand{\Vtilrep}{V}
\newcommand{\Vtildel}{\widetilde{V}_{\mathrm{del}}}
\newcommand{\Vdeli}{V^{\backslash i}}
\newcommand{\deli}{^{\backslash i}}
\newcommand{\delone}{^{\backslash 1}}
\newcommand{\delik}{^{\backslash i,k}}
\newcommand{\delk}{^{\backslash k}}
\newcommand{\delj}{^{\backslash j}}
\newcommand{\repjdeli}{^{(j) \backslash i}}
\newcommand{\Vrepi}{V^{(i)}}
\newcommand{\rep}{\mathrm{Rep}}
\newcommand{\rem}{\mathrm{Rem}}
\newcommand{\Ddeli}{D^{\backslash i}}
\newcommand{\vhis}{\wh{v}_S^{\mathrm{IS}}}
\newcommand{\vhwis}{\wh{v}^{\mathrm{WIS}}}
\newcommand{\vhwisSdel}{\wh{v}^{\mathrm{WIS}}_{\Sdel}}
\newcommand{\vhwislSdel}{\wh{v}^{\mathrm{WIS}}_{\Sdel,\lambda}}
\newcommand{\vwis}{v^{\mathrm{WIS}}}
\newcommand{\fwa}{f^{\mathrm{WA}}}
\newcommand{\Vwa}{V^{\mathrm{WA}}}
\newcommand{\WISl}{$\mathrm{WIS}_{\lambda}$}
\newcommand{\vhwisl}{\wh{v}^{\mathrm{WIS}}_{S,\lambda}}
\newcommand{\vwisl}{v^{\mathrm{WIS}}_{\lambda}}
\newcommand{\WIS}{^{\mathrm{WIS}}}
\newcommand{\wa}{^{\mathrm{\scshape{wa}}}}
\newcommand{\barf}{\bar{f}}
\newcommand{\conf}{x}
\newcommand{\param}{{\theta}}
\newcommand{\paramS}{{\tilde \theta}}
\newcommand{\ps}{\wh{p}_S}
\newcommand{\pz}{\wh{p}_z}
\newcommand{\leqC}{\lesssim}
\newcommand{\geqC}{\gtrsim}
\newcommand{\leqCln}{\lessapprox}
\newcommand{\VES}{V^{\mathrm{ES}}}
%\newcommand{\alg}{A_{S,T}}
%\newcommand{\algmap}{A}
\newcommand{\alg}{\sA_S}
\newcommand{\algloo}{\sA_{S\delk}}
\newcommand{\algmap}{\sA}
\newcommand{\Lh}{\hat{L}}



% \newcommand{\check}{\textcolor{OliveGreen}{\ding{16}}}

% ESTIMATORS and ALGORITHMS ------------------------------------

\newcommand{\hvar}{h^{\textsc{var}}}
\newcommand{\hbias}{h^{\textsc{bias}}}
\newcommand{\biasUCB}{\texttt{BiasUCB}}
\newcommand{\biasOFUL}{\texttt{BiasOFUL}}
\newcommand{\mUCB}{\texttt{MetaUCB}}
\newcommand{\mTS}{\texttt{MetaTS}}
\newcommand{\ucb}{\texttt{UCB}}
\newcommand{\ts}{\texttt{TS}}


% THEOREMS -------------------------------------------------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}{Definition}[section]
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{assumption}[theorem]{Assumption}

\newcommand{\bmid}{\;\middle|\;}
%\newcommand{\Bphi}{B_{\phi'}}
\newcommand{\Bphi}{\|\phi'\|_{\infty}}
%\newcommand{\Lphi}{L_{\phi'}}
\newcommand{\Lphi}{\|\phi''\|_{\infty}}
\newcommand{\lmaxK}{\lmax\pr{\tfrac1n \bX\tp \bX}}
\newcommand{\lminK}{\lmin\pr{\tfrac1n \bX\tp \bX}}
\newcommand{\BR}{\text{BR}}
\newcommand{\Borel}{\mathrm{Borel}}
\newcommand{\pmeta}{p^{\mathrm{meta(n)}}}
\newcommand{\bhtheta}{\boldsymbol{\hat{\theta}}}
